Semi-Supervised Laplace Learning on Stiefel Manifolds

Motivated by the need to address the degeneracy of canonical Laplace learning algorithms in low label rates, we propose to reformulate graph-based semi-supervised learning as a nonconvex generalization of a \emph{Trust-Region Subproblem} (TRS). This reformulation is motivated by the well-posedness of Laplacian eigenvectors in the limit of infinite unlabeled data. To solve this problem, we first show that a first-order condition implies the solution of a manifold alignment problem and that solutions to the classical \emph{Orthogonal Procrustes} problem can be used to efficiently find good classifiers that are amenable to further refinement. To tackle refinement, we develop the framework of Sequential Subspace Optimization for graph-based SSL. Next, we address the criticality of selecting supervised samples at low-label rates. We characterize informative samples with a novel measure of centrality derived from the principal eigenvectors of a certain submatrix of the graph Laplacian. We demonstrate that our framework achieves lower classification error compared to recent state-of-the-art and classical semi-supervised learning methods at extremely low, medium, and high label rates.

==> cover_letter.tex <==
Dear Editor,

We are submitting ``Semi-Superivsed Laplacian Learning on Stiefel Manifolds'' for consideration by the Journal of Machine Learning Research. In this paper, we motivate a semi-supervised variation of the classic Laplacian Eigenmaps framework for graph-based semi-supervised learning. In particular, our novel formulation is ideally suited to semi-supervised classification in the low-label rate regime, where classic methods based on Laplace regularized learning are ill-posed.

Our well-posed formulation, however, leads to a non-convex optimization problem (a quadratic minimization problem on the Stiefel Manifold, a non-convex set). We adapt and generalize a classic algorithm, the Sequential Subspace Method, originally designed for sphere-constrained optimization in $\mathbb{R}^n$ and show that solutions found by this technique are provably superior to those found by other methods (e.g., gradient descent) and demonstrate superior classification results at low-label rates. We further show that our algorithmic framework naturally facilitates a principled technique for active learning that comes ``for free'' (in a computational sense). 

We believe that this work is a good fit for the Journal of Machine Learning Research because it (1.) motivates and proposes a new framework for semi-supervised and active graph-based learning, derived from a well-posed problem, and associated algorithm and (2.) presents superior performance in experiments across low, intermediate and high label regimes compared to classical and state-of-the-art approaches. 

We confirm that this work is original and has not been published elsewhere, nor is it under consideration for publication elsewhere. For the role of action editor, we recommend Marco Cuturi, Shiqian Ma, and Peter Richtárik. For the role of reviewer, we suggest 
Nicolas Garcia Trillos, Luca Zanetti, Guy Wolf, and Bart Vandereycken.

Thank you for your consideration.

Sincerely,

Authors

==> figures/harmonic_example_icml.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[b]{0.49\linewidth}
\includegraphics[width=\linewidth]{figures/laplace_mnist_barcode3.png}
\subcaption{}
\label{fig:a}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/laplace_mnist_27_3.png}
\subcaption{}
\label{fig:b}
\end{subfigure}

\vspace{.1cm}

\begin{subfigure}[b]{0.49\linewidth}
\includegraphics[width=\linewidth]{figures/proc_mnist_barcode3.png}
\subcaption{}
\label{fig:c}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/proc_mnist_27_3.png}
\subcaption{}
\label{fig:d}
\end{subfigure}

\vspace{.1cm}

\begin{subfigure}[b]{0.49\linewidth}
\includegraphics[width=\linewidth]{figures/ssm_mnist_barcode3.png}
\subcaption{}
\label{fig:e}
\end{subfigure}
\begin{subfigure}[b]{0.47\linewidth}
%\includegraphics[width=\linewidth]{figures/ssm_mnist_27.png}
\includegraphics[width=\linewidth]{figures/ssm_mnist_27_2.png}
\subcaption{}
\label{fig:f}
\end{subfigure}

%
%\vspace{-0.5cm}
\caption{Barcode plots of MNIST predictors (left) and embeddings of samples for digits `2' and `7' (right).
Learning is performed with 1 label per class. 
In the barcode plots, the rows are the samples, ordered by their class. Ordering of the columns was obtained by iteratively sorting the columns of the embedding matrices $X$. (\textbf{\subref{fig:a}\textemdash\subref{fig:b}}) Laplace learning exhibits degeneracy in the limit of unlabeled data. (\textbf{\subref{fig:c}\textemdash\subref{fig:d}}) Embeddings derived using Procrustes Analysis (Section~\ref{sec:approx}) demonstrates no degeneracy but mixed samples form different classes together. (\textbf{\subref{fig:e}\textemdash\subref{fig:f}}) Our method exhibits good classification performance (a block diagonally dominant barcode) while respecting the geometry of unlabeled examples.}
\label{fig:mnist}
\end{figure}

==> figures/projection_icml.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.498\linewidth}
\resizebox{4cm}{4cm}{\scalebox{1.0}[1.0]{\reflectbox{\includegraphics[width=\linewidth]{figures/barbell/barbell_ev4.png}}}}
\subcaption{}
\label{fig:grid1}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\resizebox{4cm}{4cm}{\scalebox{1.0}[1.062]{\includegraphics[width=\linewidth]{figures/barbell/barbell_refine4.png}}}
\subcaption{}
\label{fig:grid2}
\end{subfigure}

\vspace{.1cm}

\begin{subfigure}[b]{0.498\linewidth}
\resizebox{4cm}{4cm}{\scalebox{1.0}[1.0]{\includegraphics[width=\linewidth]{figures/barbell/barbell_labeled4.png}}}
\subcaption{}
\label{fig:grid3}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\resizebox{4cm}{4cm}{\scalebox{1.0}[1.062]{\includegraphics[width=\linewidth]{figures/barbell/barbell_transformed4.png}}}
\subcaption{}
\label{fig:grid4}
\end{subfigure}

%
%\vspace{-0.5cm}
\caption{\textbf{Eigenvector method and projection example on the barbell graph}. (\textbf{\subref{fig:grid1}}): Embedding via Laplacian Eigenmaps. (\textbf{\subref{fig:grid2}}): Several iterations of gradient-based repulsion are applied to remove vertex overlaps for better visualization.
(\textbf{\subref{fig:grid3}}): Consider taking an arbitrary vertex from each clique and assigning it a label (green vertices) such that the embedding is \emph{inconsistent} with the labels. (\textbf{\subref{fig:grid4}}): Orthogonal transform $Q$ derived from Prop. \ref{rem:negdef} and applied to $X$; $XQ$ resolves the discrepancy between the embeddings and the labeled vertices.}
\label{fig:procrustes}
\vspace{-0.25cm}
\end{figure}

==> sections/max_small_eigenvalue_stuff.tex <==
Let the smallest eigenvalue $\lambda(\mathcal{U})$ of a grounded Laplacian matrix $L_\mathcal{U}$. Previously, it was shown that $\lambda(\mathcal{U})$ is a monotonic increasing function of $u$ as a consequence of interlacing. Formally, we aim to find a subset $u \subseteq \mathcal{V}$ with $0 < m \ll M$ so that the smallest eigenvalue of the grounded Laplacian matrix $L_\mathcal{U}$ is maximized. 

\begin{equation}
u^* = \argmax_{\mathcal{U} \subseteq \mathcal{V}, |\mathcal{U}| = M} \lambda(\mathcal{U})
\label{eq:eigenvalue_opt}
\end{equation}

Equation~\ref{eq:eigenvalue_opt} is a combinatorial optimization problem. Solving directly by enumerating $u$ is not feasible for large benchmarks.

%The first algebraic landmarking method~\cite{Xu2015ActiveML} minimized an algebraic reconstructed error bound based on Gershgorin circle theorem~\cite{}. However, this method suffers from high complexity due to logarithmic computations of a large matrix. Recently,~\cite{} introduced a fast unified strategy to combine geometric and algebraic methods for landmarking, but exhibits has sub-par performance due to many relaxations. 
In this section, we propose a straightforward lower-bound on the smallest eigenvalue motivated by the decomposition derived in Section~\ref{sec:formulation}. In particular the observation that the decomposition of the Laplacian, $\mathcal{L}$ described in Section \ref{sec:formulation} implies an active learning scheme which perturbs the original graph by removing labeled vertices and reconnecting incident edges to the neighborhood of the labeled nodes. The associated perturbation to the eigenvalues can be derived by examining a transformation of the rayleigh quotient of $L_\mathcal{U}$. 

Let $L$ be a Laplacian matrix. Let $L_\mathcal{U}$ be the grounded Laplacian matrix for some unlabeled vertex set $\mathcal{U}$ with $n$ elements. Let $\mathcal{U}^c$ be the complement of $\mathcal{U}$, i.e., $\mathcal{U}^c$ consists of $m$ labeled vertices. Let $\lambda(\mathcal{U})$ be the smallest eigenvalue of $L_\mathcal{U}$. That is,
$$
\lambda(\mathcal{U}) = \min\{\frac{u^\top L u}{||u||^2}\:\: |\:\: \text{supp}(u) \subset \mathcal{U},\:\: u \in \mathbb{R}^n\}
$$
We then intend to solve the following:
$$
\max_u \{\lambda(\mathcal{U})\:\: |\:\: |\mathcal{U}^c| = m\}
$$
Suppose that $\mathcal{U}^c$ is some optimal set with cardinality $m - 1$. We will extend the set $\mathcal{U}^c$ to $\mathcal{U}^c \cup \{i\}$ by adding (removing) vertex $i$ to $\mathcal{U}^c$ ($\mathcal{U}$), where the selection is based on a lower bound estimate.

\iffalse
For simplicity, let $u$ be one unit eigenvector of $L_\mathcal{U}$ corresponding to the smallest eigenvalue $\lambda(\mathcal{U})$. Consider the extension $\mathcal{U} \to \mathcal{U}_i' := \mathcal{U} \setminus \{i\}$ with some $i \in \mathcal{U}$. Let $1_i \in \mathbb{R}^n$ be an indicator vector with single nonzero at the $i$-th component. Introduce $u' := u \odot (1 - 1_i)$, which eliminates the $i$-th entry in $u$. Then for each $i \in \mathcal{U}^c$, the eigenvalue $\lambda(\mathcal{U} \setminus \{i\})$ has a lower bound,
\begin{equation}
\begin{aligned}
\lambda(\mathcal{U} \setminus \{i\}) &\geq \frac{u'^\top Lu'}{||u'||^2} \geq u'^\top L u' \\ 
%\lambda(\mathcal{U} \setminus \{i\}) &\geq \lambda(\mathcal{U}) = \frac{u^\top  L_\mathcal{U}u}{||u||^2} = u^\top L_\mathcal{U} u \geq u'^\top  L_\mathcal{U} u' \\ 
&= u^\top  L_\mathcal{U} u - 2\sum_{j \in \mathcal{U}} (L_\mathcal{U})_{ij}u_j u_i- (L_\mathcal{U})_{ii}u_i^2 \\
&= \lambda(\mathcal{U}) + 2u_i \sum_{j \in \mathcal{U}} A_{ij}u_j - D_{ii}u_i^2
\end{aligned}
\end{equation}
Hence, the increase of the smallest eigenvalue is at least $2u_i \sum_{j \in \mathcal{U}} A_{ij}u_j - D_{ii}u_i^2 \geq 2u_i \sum_{j \in \mathcal{U}} A_{ij}u_j - \gamma D_{ii}u_i^2$, for some parameter $\gamma \in [0,1]$ when the vertex $i$ is added to $u$. The follow proposition provides a geometric interpretation of the lower-bound when $\gamma=0$. This choice of $\gamma$ is motivated by the following observation, which is consistent with the intuition that selecting nodes with large degrees is a good solution when only choosing a few number of labeled nodes.
\fi
%\subsection{Perturbation analysis}

If we have $L' = L + E$, then if $\lambda$ is an eigenvalue of $L$, the corresponding $\lambda' $of $L'$ can be expressed as $\lambda' = \lambda + \delta \lambda^{(1)} + \delta^2 \lambda^{(2)} + \ldots$ where $\lambda^{(i)}$ are eigenvalues of other matrices.

Weyl's inequality also states a corresponding lower bound: $\lambda (L + E) \geq \lambda (L) + \lambda_\text{min}(E)$

Consider a grounded Laplacian $L_\mathcal{U}$. If an edge $e = (v_i, v_j)\in E$ such that $v_i, v_j \in \mathcal{U}$ is removed, the resulting Laplacian can be represented by $L + E_{ij} + E_{ji}$. Let $\Delta L_\mathcal{U} = (E_{ij} + E_{ji})$ and consider the perturbation:
%
$$
(L_\mathcal{U} + \Delta L_\mathcal{U})(u + \Delta u) = (\lambda + \Delta \lambda)(u + \Delta u)
$$
%
Multiply both sides by $u^\top$ and eliminate the common terms. It follows that
%
$$
u^\top \Delta L_\mathcal{U} u + u^\top \Delta L_\mathcal{U} \Delta u = u^\top \Delta \lambda u + u^\top \Delta \lambda \Delta u,\implies 
\Delta \lambda = \frac{u^\top \Delta L_\mathcal{U} \hat{u}}{u^\top \hat{u}} = \frac{u_i\hat{u}_j + u_j \hat{u_i}}{u^\top \hat{u}}
$$
%
where $\hat{u} = u + \Delta u$. In the limit, note that $\Delta u \approx 0$, so $\Delta \lambda \approx 2u_i u_j$. summing over all edges incident to vertex $i$ yields the perturbation $\Delta \lambda \approx 2\cdot u_i \sum_{v_j \in \mathcal{U}}A_{ij}u_j$.

\iffalse
\begin{proposition}[Smallest eigenvalue of $L_\mathcal{U}$]
For the matrix $L_\mathcal{U}$, w define ($(\lambda, u)$ to be an eigenpair corresponding to the smallest eigenvalue $\lambda$ and its associated eigenvector $u$. for the grounded Laplacian matrix $L_\mathcal{U}$. For any vertex $i \in V \setminus l$, define $\Delta L_\mathcal{U} = \sum_{j\in N_i \setminus l}(E_{ij} + E_{ji})$. Additionally, we define the \emph{neighborhood} of a vertex $v_i$ $N_i$ to be the set $\{v_j\}$, s.t. $A_{ij} = 1$, i.e. those vertices which share an edge with $v_i$. For the case where $L_\mathcal{U}$ is perturbed by $\Delta L_\mathcal{U}$, suppose $\lambda$ varies with $\Delta \lambda$ and $u$ varies with $\Delta u$. Then
$$
(L_\mathcal{U} + \Delta L_\mathcal{U})(u + \Delta u) = (\lambda + \Delta \lambda) (u + \Delta u)
$$
and the eigen-gap for the smallest eigenvalue can be approximated by 
$$
\Delta \lambda \approx 2\cdot u_i \sum_{v_j \in \mathcal{U}}A_{ij}u_j
$$
\end{proposition}
\fi


==> sections/method_backup.tex <==
\subsection{Semi-supervised spectral learning algorithms}
\label{sec:algorithms}

In this section, we introduce approximate and iterative methods to solve \eqref{eq:rescaled_f}. 
In theory, as we show in the appendix, one can start with an arbitrary initialization to obtain a critical point of \eqref{eq:rescaled_f} using a variety of projection- or retraction-based gradient methods, with the descent direction given by the gradient of \eqref{eq:rescaled_f} and projection given by \eqref{rem:stiefel_projection}. However, the empirical rate of convergence depends significantly on the initialization of the embedding matrix $X$.
In order to improve convergence of our method, we first introduce and motivate an efficient method based on Procrustes Analysis~\cite{wang08manifold} to approximately compute critical points of the \emph{unscaled} objective ($C = I$).
This approximation is appropriate in the limit of few labeled examples or unlimited unlabeled data: 
since $C = (p-\widetilde{p})I - \frac{\tilde{p}^2}{n}\mathbf{1}\mathbf{1}^\top$, then $C \to pI$ in the limit of $\frac{m}{n} \to 0$.

%\chester{This approximation is motivated by the observation that . Since . In the limit, as $n\to \infty$, $C \to pI$.}

\subsection{Efficient approximation via Orthogonal Procrustes}
\label{sec:approx}
%
Here we propose an efficient way to compute approximate critical points of \eqref{eq:rescaled_f}. First we solve the canonical eigenvalue problem $\min_X \text{tr}(X^\top LX)$ subject to a constraint on the second moment of $X$: $X^\top X = I$, yields $X$ are the eigenvectors of $L$.
%(2.) invoking a projection to resolve the second-order constraint $X^\top X = C$; 
Second, we appropriately transform the solution so that $X^\top B$ is positive definite (i.e. satisfies a necessary condition for first-order optimality). 
\begin{proposition}[Definiteness conditions of $X^\top B$]
Assume $C = I$. Note the first term of the objective in \eqref{eq:rescaled_f} satisfies the invariance $\langle X, LX\rangle = \langle \widetilde{X},  L\widetilde{X}\rangle$, where $\widetilde{X} = XQ$ for any orthogonal $Q \in \mathbb{R}^{k\times k}$. Suppose $X$ is a local minimizer of \eqref{eq:rescaled_f}. Then, $X^\top B\succcurlyeq 0$ and symmetric. 
\label{rem:negdef}
\end{proposition}
%
\emph{Proof.} Note that by assumption, $X$ is feasible\textemdash i.e. $X^\top X = I$. Consider the substitution $X \to XQ$ for some orthogonal matrix $Q$. Since $C = I$, $F(XQ) = \langle XQ, LXQ \rangle - \langle Q, X^\top B \rangle$.

Fix $X$. Note that the first term satisfies the invariance $\langle X, LX \rangle = \langle XQ, LXQ \rangle$. For any orthogonal $Q \in \mathbb{R}^{k\times k}$. The optimal choice of $Q$ is determined by the second term. A standard result from matrix analysis yields its minimizer~\cite{horn13}. Let $X^\top B = UDV^\top$ be the SVD of $X^\top B$. Then, $Q = U_B V_B^\top$ and $\langle XQ, B\rangle = \langle Q, X^\top B \rangle = \langle I, D \rangle = tr(D) \geq 0$. \hfill\qedsymbol

A consequence of this is the following: Let the SVD of $X^\top B = U_BD_BV_B^\top$ and let $Q = U_BV_B^\top$. 
%Then $\text{tr}((XQ)^\top B) = -\text{tr}(D_B) \leq 0$. 
Algorithmically, this implies that projecting $X$ onto $Q$ decreases the objective of \eqref{eq:rescaled_f} (assuming $C=I$). Note, in practice, we can additionally rescale predictions by taking $X\gets XC^{1/2}$ to properly observe the constraint on the second moment of $X$.  %\\

This step can be interpreted as an alignment step, where we find an orthogonal transformation $Q$ that aligns unlabeled vertices with their neighboring labeled vertices, and apply this transformation to all unlabeled vertices.  
We briefly describe the connection with Orthogonal Procrustes Analysis~\cite{wang08manifold}. Let $X$ be feasible, i.e. $X^\top X = I$. Note that the invariance is nothing but $\text{tr}(X^\top L X) = \langle X, LX \rangle = \langle XQ, LXQ \rangle$ for any orthogonal $Q$. Thus, 
%
\iffalse
\begin{equation}\label{eq:procrustes}
\begin{aligned}
&\argmin_{Q : Q^\top Q = I}\langle XQ, LXQ \rangle - \langle XQ, B \rangle \\
=&\argmax_{Q : Q^\top Q = I} \langle XQ, B \rangle \\
=&\argmin_{Q : Q^\top Q = I} ||XQ - B||^2_F. \\
\end{aligned}
\end{equation}
\begin{equation}\label{eq:procrustes}
\begin{aligned}
&\argmin_{Q :Q\in \textrm{St}(k,k)}\langle XQ, LXQ \rangle - \langle XQ, B \rangle \\
=&\argmax_{Q :Q\in \textrm{St}(k,k)} \langle XQ, B \rangle \\
=&\argmin_{Q :Q\in \textrm{St}(k,k)} ||XQ - B||^2_F. \\
\end{aligned}
\end{equation}
\fi
\begin{equation}\label{eq:procrustes}
\begin{aligned}
\argmin_{Q :Q\in \textrm{St}(k,k)}\langle XQ, LXQ \rangle - \langle XQ, B \rangle 
=\argmax_{Q :Q\in \textrm{St}(k,k)} \langle XQ, B \rangle 
=\argmin_{Q :Q\in \textrm{St}(k,k)} ||XQ - B||^2_F. 
\end{aligned}
\end{equation}
%
This problem is the canonical Orthogonal Procrustes problem in $\mathbb{R}^{k\times k}$ in the context of finding an alignment between the axis-aligned labeled vertices and their neighborhood of unlabeled vertices. We demonstrate the effect of this procedure in Figure~\ref{fig:procrustes}. In Figure~\ref{fig:procrustes}\subref{fig:grid1}\textemdash\subref{fig:grid2}, we plot the first pair of eigenvectors corresponding to the smallest two nonzero eigenvalues associated with a barbell graph. In Figure~\ref{fig:procrustes}\subref{fig:grid3}, we pick a random pair of vertices $v_i$ and $v_j$ with coordinates $x_i$ and $x_j$ from each clique and assign labels $y_i = x_i$ and $y_j = x_j$. Under this labeling, we say that the embedding is \emph{inconsistent}. In other words, a linear predictor in the space spanned by the embedding would be incapable of recovering a separating hyperplane that accurately classifies the unlabeled samples. We then show that by applying the approximate method based on Procrustes Analysis introduced in Section \ref{sec:approx}, we recover an embedding which is \emph{consistent} with the labels.
%
\input{figures/projection.tex}
%
%\input{figures/harmonic_example.tex}

Alternatively, the projection and $Q$-transform
%solving the first-order condition \eqref{eq:rescaled_f_foc} 
%
%corresponds to performing the following pair of steps: (1.) first calculating the rescaled eigenvectors of $L$ (2.) finding an orthogonal transform to align vertex labels via supervision. This procedure 
%
can be interpreted as 
%finding the solution to a linear alignment problem, i.e. solving an Orthogonal Procrustes Problem~\cite{wang08manifold} by 
performing orthogonal multivariate regression in the space spanned by the first $k$ nontrivial eigenvectors of $L$: 
$$
%Q = \argmin_{Q:Q^\top Q = I}\sum_{i\in [m]}||x_iQ - y_i||_2^2, 
Q = \argmin_{Q :Q\in \textrm{St}(k,k)}\sum_{i\in [m]}||x_iQ - y_i||_2^2, 
$$
where $Q \in \mathbb{R}^{k\times k}$ and predictions are given by $XQ$. Note that this is similar in principal to the Semi-Supervised Laplacian Eigenmaps (SSL) algorithm~\cite{Belkin2002UsingMS}, which solves an ordinary least squares problem using eigenvectors $X$ of the Laplacian as features:
$$
Q = \argmin_{Q}\sum_{i\in [m]}||x_iQ - y_i||_2^2.
$$
Crucially, the orthogonality constraint on $Q$ ensures that the solution remains feasible, i.e. that $XQ \in \text{St}(n,k)$. Furthermore, we show in our experiments that this feasability significantly improves generalization at very low label rates in comparison to standard Laplacian Eigenmaps SSL.
These interpretations serve to motivate our initialization and subsequent refinement. In particular, \citet{zhou2011error} consider the limiting behavior of Laplacian Eigenmaps SSL and show that it is non-degenerate in the limit of infinite unlabeled data.

\subsection{Iterative refinement with SSM and KL}
To refine solutions produced by the Procrustes algorithm into solutions to \eqref{eq:rescaled_f}, we introduce an efficient iterative method capable of global convergence to high-quality stationary points. Motivated by the similarity between \eqref{eq:rescaled_f} and standard trust-region subproblems, we develop the framework of the \emph{Sequential Subspace Method (SSM)}. In the $k=1$ and $C=I$ case, SSM has been applied to Trust-Region sub-problems with remarkable empirical results~\cite{Hager2001MinimizingAQ} and robust global convergence guarantees~\cite{Hager2005GlobalSSM}, even for so-called degenerate problems. SSM-based algorithms generate a sequence of iterates $X_t$ by solving a series of rescaled quadratic programs (of the same form as \eqref{eq:rescaled_f}) in subspaces of dimension much smaller than that of the original problem (where $d = |V|$, the number of vertices in the graph).  

Although stationary points can be recovered via generic iterative project-descent procedures\textemdash gradient-based or Newton-based descent directions (e.g. via SQP or trust-region-type algorithms), SSM is a computationally friendly algorithm designed to address scalability with respect to large problems. We develop a SSM on the Stiefel manifold, which is inspired by the $1$-dimensional algorithm of \cite{Hager2001MinimizingAQ}, originally proposed to solve large trust-region subproblems. %In other words, instead of solving \eqref{eq:cneqi} directly as previously mentioned, we instead solve a sequence of quadratic programs in subspaces of much smaller dimension relative to the size of the graph (the dimensions of $L$). 

At step $t$ a tiny subspace, $S_t$, of dimension $4k$ is derived from the current iterate $X_t$, the gradient of the objective of \eqref{eq:rescaled_f} $g_t=LX_tC - BC^{1/2}$, an \emph{SQP} (i.e. Newton's method applied
to the first-order optimality system $X_t$) iterate $X_{\text{sqp}}$ derived in Prop.~\ref{prop:newton}, and the principal eigenvectors of $L$. The Sequential Quadratic Programming (SQP) framework~\cite{nocedal99sqp} is adapted to compute $X_{\text{sqp}}$. $X_{t+1}$ is then generated by solving \eqref{eq:rescaled_f} in this small subspace. 
%
\iffalse
SSM generically involves repeating the following pair of steps:
%
\begin{enumerate}
    \item Compute the SQP direction $Z = \text{SQP}(L,\Lambda, B, X)$ as defined in Prop.~\ref{eq:sqp} and Alg.\ref{alg:sqp}, line 5.  Let $V$ be the orthogonal matrix consisting of columns in $S$ (Alg.\ref{alg:ssm}, lines 6 and 7), where
    $$
    S = \text{span}(X_t, Z_t, u, g_t).
    $$
    \item SSM generates an approximation of $(X,\Lambda)$ and an approximation of the smallest pair of eigenvalues $\sigma$ and eigenvectors $u$ of $L$ in the subspace $S$,
    $$
    [X,\Lambda, u, \sigma] = \text{SSM}(L, B, S)
    $$
    consider the approximation $X = V \widetilde{X}$ for some $\widetilde{X}$. Compute
    \begin{equation}
    \min_{\widetilde{X} \in \text{St}(\widetilde{n},k)}F_{S} := \min_{\widetilde{X}}F(\widetilde{X}; V^\top L V, V^\top B).
    \label{eq:subspace_prob}
    \end{equation}
    %We can consider $v = V\tilde{v}$ to be a matrix consisting of estimates of the eigenvectors of $L$, if $\tilde{v}$ corresponds to a pair of eigenvectors of $B$ associated with its smallest two nontrivial eigenvalues (Alg.\ref{alg:sqp}, line 9).
\end{enumerate}
%
Note that \eqref{eq:subspace_prob} is solved using the Projected Gradient Method, where the projection is given by \cref{rem:stiefel_projection}: $[X]_+ = UV^\top$. %, where $U$ and $V$ are given by the singular value decomposition; $U\Sigma V^\top = \text{SVD}(X)$. 
We update $\Lambda$ according to the least-squares estimate derived from the first order condition in \eqref{eq:rescaled_f_foc} $\Lambda = X^\top (AXC - BC^{1/2})$.
\fi
%
Crucially, we highlight that when the eigenvectors of $L$ are included in the subspace, the sequence of iterates generated by SSM exhibits the following global convergence property, which we discuss further in the appendix. 

\input{statements/ssm_convergence.tex}

To further adjust predictions, we introduce a multi-class Kernighan-Lin (KL) refinement algorithm to iteratively adjust the classification to improve a cut-based cost. Critically, this method is efficient (linear-time) and, in contrast to the gradient-based refinement method proposed in PoissonMBO~\cite{calder20poisson}, robust to the nonconvexity of the cut objective.

\section{Algorithms for Graph-Based Semi-Supervised Learning}

\subsection{Preliminaries}
\begin{equation}\label{eq:rescaled_f_apdx}
\begin{aligned}
\min_{X :X\in \textrm{St}(n,k)} \langle X, L X C \rangle - \langle X, B C^{1/2} \rangle
\end{aligned}
\end{equation}
Quadratic minimization over the Stiefel manifold is a generalization of the well-known nonconvex quadratic over the unit ball or sphere. These problems often arise in trust region methods \cite{sorensen82newtontrust, conn00trust}. Notably, there could exist many local solutions in \ref{eq:rescaled_f_apdx}. We will demonstrate convergence to critical points of two iterative methods: a gradient projection method and the Sequential Subspace Method proposed in this work. Furthermore, when the subspaces component to the SSM algorithm contain the span of the first $k$ nontrivial eigenvectors of $L$, we show that the quality of the stationary point is characterized by the eigenvalues of the Lagranage multipliers $\Lambda$.

First denote the the eigenvector decomposition of $L$ be given by
$$
L = [v_1, v_2, \ldots, v_n]\text{diag}(d_1, \ldots, d_n)[v_1, v_2, \ldots, v_n].T
$$

To summarize, we will show the following:
\begin{itemize}
    \item We propose a gradient projection method to solve \ref{eq:rescaled_f_apdx}. We prove convergence with the Armijo rule in Prop.~\ref{prop:pgd_convergence}.
    \item We analyze the proposed iterative method in the framework of SSM, constructing a sequence of subspaces to reach one approximation of local solutions, where the subspace consists of columns of $X_t$, $LX_tC-BC^{1/2}$ and eigenvectors associated with $d_i$, $i=1,\ldots,k$. Each sub-problem can be solved by the aforementioned gradient projection method. We demonstrate global convergence to high-quality critical points. Theoretically, when $C=I$ and the multiplicity of the first nontrivial eigenvalue is greater than or equal to $k$, a local solution is actually a global solution. However, we leave this analysis as future work.
\end{itemize}
First, we review some known results in the spherical case, i.e., $\text{St}(n, 1)$. Next, we derive convergence of a projected gradient method to solutions satisfying the first order condition~\eqref{eq:rescaled_f_foc}. Finally, Theorem 1 states the convergence of SSM to a high-quality local solution is guaranteed.

\subsubsection{Notation}

We assume $k$ is a positive integer (much) less than $n$. Let $K$ denote the set $\{1, 2,\ldots , k\}$. Let $I_{n,k}$ denote the sub matrix of the identity matrix $I_n$, consisting of the first $k$ columns. Let $O_k$ be the orthogonal group, i.e., $Q \in O_k$ if and only if $Q \in \mathbb{R}_{k,k}$ and $Q^\top Q = I_k$.

\subsection{Preliminary results in the spherical case}
\eqref{eq:rescaled_f_apdx} is one natural generalization of the constrained problem \cite{Hager2001MinimizingAQ,Hager2005GlobalSSM}
\begin{equation}\label{eq:hager}
\min_x \{x^\top A x - 2\langle x, b\rangle: ||x|| = 1, x\in \mathbb{R}^n\}
\end{equation}
This problem is related to the trust region subproblem:
\begin{equation}\label{eq:trust}
\min_x \{x^\top A x - 2\langle x, b\rangle: ||x|| \leq 1, x\in \mathbb{R}^n\}
\end{equation}
The following two propositions describe the global solution of \ref{eq:hager}. See \cite{sorensen82newtontrust}. The condition \ref{eq:trust_opt_condition} states that the global solution $x$ is the critical point associated with $\lambda$ bounded above by the smallest eigenvalue $d_1$ of $A$.
%
\begin{proposition}[\citet{Hager2005GlobalSSM}]
A vector $x \in \mathbb{R}^n$ is a global solution of \ref{eq:hager}, if and only if $||x|| = 1$, and
\begin{equation}\label{eq:trust_opt_condition}
A - \lambda I \succcurlyeq 0, \:\: (A - \lambda I)x = b
\end{equation}
holds for some $\lambda \in \mathbb{R}$
\label{prop:global_solution}
\end{proposition}
%
\begin{proposition}[\citet{Hager2001MinimizingAQ}]
Consider the eigenvector decomposition 
$$
A = [v_1, v_2, \ldots, v_n]\text{diag}(d_1, \ldots, d_n)[v_1, v_2, \ldots, v_n].T.
$$
Let $V_1$ be the matrix whose columns are eigenvectors of $L$ with eigenvalue $d_1$. Then, $x = Vc$ is a solution for a vector $c$ chosen in the following way:
\begin{itemize}
\item Degenerate case: suppose $V_1^\top b = 0$ and $c_{\perp}:= ||(A - d_1I)^{\dagger}b||\leq 1$
Then, $\lambda = d_1$ and $x = (1 - c_\perp^2)^{1/2}v_1 + (A - d_1 I)^{\dagger} b$
\item Nondegenerate case: $\lambda < d_1$ is chosen so that $x = (A - \lambda I)^{-1}b$ with $||x|| = 1$.
\end{itemize}
\label{prop:plp}
\end{proposition}
%
\begin{remark}[\citet{Hager2005GlobalSSM}]
Note that $||(A - \lambda I)^{-1}b||$ decreases monotonically with respect to $\lambda\leq d_1$. A proper value of $\lambda$ meets the condition $||x|| = 1$. A tighter bound on $\lambda$ can be estimated from 
$$
(d_1 - \lambda) ||V_1b||^2 \leq 1 = ||(A - \lambda I)^{-1}b||^2 \leq (d_1 - \lambda)^{-2}||b||^2
$$
With $||V_1 b|| > 0$, $\lambda$ lies in the interval $[d_1 - ||b||, d_1 - ||V_1 b||]$
\label{prop:plp}
\end{remark}

Several of the algorithms we describe necessitate computation of pseudoinverse-vector products of the perturbed Laplacian $PL_\mathcal{U}P$\textemdash i.e. $(PL_\mathcal{U}P)^{\dagger}u$. Here, we demonstrate that the computation of $(PL_\mathcal{U}P)^{\dagger}u$ is computationally comparable to computing a standard laplacian pseudoinverse-vector product, $L_\mathcal{U}^{\dagger}u$, for which there exist nearly linear-time solvers~\cite{spielmanteng}.
\begin{proposition}[Psudo-inverse of $PL_\mathcal{U}^{-1}P$]
Let $P = I - vv^\top$ for a unit vector $v$. Let $r_k = \{PL_\mathcal{U}^{-1}P\}^\dagger u_{k-1}$. Then, the projection of $r_k$ is
$$
Pr_k = \{PL_\mathcal{U}^{-1}P\}^\dagger u_{k-1} = (I - \frac{\bar{v}^\top v}{v^\top \bar{v}})L_\mathcal{U}^{-1}u_{k-1},\quad \bar{v} = L_\mathcal{U}^{-1}v
$$
\label{prop:plp}
\end{proposition}

\subsection{Gradient Projection Method (PGD) Algorithm}
We first introduce a projected gradient-based method. With appropriate step size $\alpha > 0$, PGD produces iterates $X_t$, $t = 1, 2, \ldots$
$$
X_{t+1} = [X_t - \alpha g_t]_+
$$
Where $g_t$ is given by the gradient of the objective of \eqref{eq:rescaled_f_apdx}\textemdash i.e. $g_t = LX_tC - BC^{1/2}$ and $[X_t]_+$ is the projection onto the manifold
$$
\mathcal{M} := \{X : X \in St(n,k), X^\top B \geq 0\}
$$
We first describe the projection $X = [X_1]_+$ as a composition of two projections; i.e. $[X_1]_+ = [[X_1]_{St}]_\mathcal{B} \in \mathcal{M}$:
\begin{flalign}
& Z = [X_1]_{St} := \argmin_Z \{||X_1 - Z||_F : Z \in St(m,r)\} \label{eq:stproj} \\
& X = [Z]_\mathcal{B}:= ZQ,\:\:Q=\argmin_Q \{||Z - BQ^\top||_F : Q \in O_k\} \label{eq:Bproj}
\end{flalign}
In other words, $Z \in St(n,r)$ and $Q \in O_k$ are chosen to minimize the sum
$$
||X_1 - Z||_F^2 + ||Z - BQ^\top||_F^2 = ||X_1Q - ZQ||^2_F + ||ZQ - B||_F^2
$$
Take the SVD of $X_1$, i.e. $X_1 = U_XD_XV_X^\top$. Then, the solution to \eqref{eq:stproj} is given by $Z = U_XV_X^\top$. Likewise, $X=ZQ$ for some orthogonal matrix $Q$ chosen to maximize $\langle X, B \rangle = X^\top B$. 

\begin{proposition}[Projection onto $\mathcal{B}$]\label{prop:projection}
Consider the solution to the following projection:
\begin{equation}\label{eq:proj_apdx}
[X_1]_+ = \argmin_{X\in St(n,k)}\{\min_Q ||X - X_1Q||_F^2 : X^\top B \geq 0, Q \in O_k\}
\end{equation}
Suppose the singular values of $X_1$ and $B$ are positive. Then, the minimizer $X$ is uniquely determined by 
$$
X = [X_1]_+ = U_1 U_2 V_2^\top
$$
where $U_1, V_1, V_2$ are determined from the two SVDs,
$$
U_1 \Sigma_1 V_1^\top = X_1, \:\: U_2\Sigma_2V_2^\top = U_1^\top B
$$
\end{proposition}
\emph{Proof.} The minimizer $X$ in \eqref{eq:proj_apdx} is the maximizer of $\max_X \langle X, X_1 Q\rangle$. Note that
$$
\langle X, X_1 Q\rangle = \langle X, U_1 \Sigma_1 V_1^\top Q \rangle = \langle U_1^\top X Q^\top V_1, \Sigma_1 \rangle \leq tr(\Sigma_1)
$$
Note two observations: (1) that $U_1^\top X Q^\top V_1$ lies in $O_k$, and (2) that equality holds if and only if $U_1^\top X Q^\top V_1 = I_k$ for some $XQ^\top V_1 \in \text{St}(n, k)$, i.e. $XQ^\top V_1 = U_1$, and thus,
$$
X = U_1 V_1^\top Q.
$$
Furthermore, the condition $X^\top B$ is symmetric and positive definite implies a choice of $Q$ that fulfills 
$$
X^\top B = Q^\top V_1 U_2 \Sigma_2 V_2^\top, \:\: i.e., V^\top Q = V_2 U_2^\top
$$
Finally, note that since the singular values $\Sigma_1, \Sigma_2$ are distinct and positive, $U_1$ and $V_1$ are uniquely determined up to column-sign $Q_1 = \text{diag} (\pm 1, \ldots \pm 1)$. Likewise, $U_2$ and $V_2$ are uniquely determined up to $Q_2 = \text{diag} (\pm 1, \ldots \pm 1)$. Hence,
$$
X = U_1 Q_1 Q_2^\top U_2 Q_2 Q_2^\top V_2^\top = U_1 U_2 V_2^\top
$$
is unique. \qedsymbol

\begin{remark}\label{rem:differential}
Consider the function $h(X) = [X]_{\text{St}}$ defined on $\mathbb{R}^{n\times k}$ and $X\in St(n,k)$. The differential $\mathbb{D}h$ at $X$ is the linear map given by
$$
\mathbb{D}h(X)[T] - \lim_{\alpha \to 0}\alpha^{-1}(h(X + \alpha T)-h(X)) = (I - XX^\top)T + (-1/2)X(T^\top X - X^\top T)
$$
for each $T\in \mathbb{R}^{n\times k}$. When $X \in \mathcal{M}$ and $T = -(LXC - BC^{1/2})$, then
$$
\langle T, \mathbb{D}h(X)[T] \rangle = ||(I- XX^\top)T||_F^2.
$$
\end{remark}

\subsection{Convergence of the Projected Gradient Method (PGD)}
The convergence of the gradient method with Armijo rule would be verified in Prop 4.5. The step size...

\begin{proposition}\label{prop:pgd_convergence}
Let $d_t = -(LX_tC - BC^{1/2})$. Let $\{X_t\}$ be a sequence generated by the gradient projection method
$$
X_{t+1} = [x_t + \alpha_t d_t]_+
$$
where $\alpha_t$ is chosen according the Armijo rule. Then, every limit point of $\{X_t\}$ is a stationary point.
\end{proposition}
\emph{Proof.} The proof is motivated by the proof by contradiction of Prop. 1.2.1 in \citet{bertsekas99nonlinprog}.

Let $\mathcal{G}(X) = (I - X^\top X)(AXC - BC^{1/2})$ be the projected gradient of the objective of \ref{eq:rescaled_f_apdx}, $F$ at $X$. We define $\alpha$ given by the Armijo rule\textemdash i.e. let $s > 0$, $\sigma \in (0,1)$ and $\beta \in (0,1)$. $\alpha_t = \beta^{m_t}s$, where $m_t$ is the first nonnegative integer $m$ for which
$$
F(X_t) - F([X_t + \beta^msd_t]_+)\geq -\sigma \beta_t s\langle \mathcal{G}(X_t), d_t \rangle
$$
Suppose $\hat{X}\in \mathcal{M}$ is a limit point of $\{X_t\}$ with $||\mathcal{G}(\hat{X}|| > 0$. By definition, $\{F(X_t)\}$  is monotonically nonincreasing to $F(\hat{X})$., i.e. $F(X_t) - f(X_{t-1}) \to 0$. By definition, since the $\alpha_t$, the step sizes are generated via the Armijo rule, $a_t$ satisfies
\begin{equation}\label{eq:armijo}
\begin{aligned}
F(X_t) - F(x_{t+1}) &\geq F(X_t) - F([X_t + \alpha_t d_t]_+) \\
&\geq -\sigma \langle \mathcal{G}(X_t), d_t \rangle = \sigma \alpha_t ||\mathcal{G}(X_t)||_F^2
\end{aligned}
\end{equation}
Let $\{X_t\}_{\mathcal{T}}$ be a subsequence converging to $\hat{X}\in \mathcal{M}$ Since 
$$
\lim_{t \to \infty} \sup -\langle \mathcal{G}(X_t), d_t \rangle = ||\mathcal{G}(\hat{X})||^2 > 0,
$$
\eqref{eq:armijo} implies $\{\alpha_t\}_{\mathcal{T}}\to 0$. From Armijo's rule, for some $t'\geq 0$, the inequality
\begin{equation}\label{eq:armijo2}
F(X_t) - F([X_t + \alpha_t \beta^{-1}d_t]_+)< -\sigma \alpha_t \beta^{-1} \langle \mathcal{G}(X_t), d_t \rangle
\end{equation}
holds for all $t \geq t'$. By taking a subsequence $\{d_t\}_{\mathcal{T}'}$ of  $\{d_t\}_{\mathcal{T}}$ such that $\{d_t\}_{\mathcal{T}'} \to d'$ and $X_t \to X'$, applying the mean value theorem to the left hand side of \eqref{eq:armijo2}, we have that
\begin{flalign*}
&-\langle L([X_t + \alpha_t' d_t]_+C) - B, \mathbb{D}([X_t + \alpha_t' d_t]_+)[d_t] \rangle \\
&=(\alpha_t \beta^{-1})^{-1}(F(X_t)) - F([X_t + \alpha_t \beta^{-1}d_t]_+) \\
&< -\sigma \langle \mathcal{G}(X_t), d_t\rangle
\end{flalign*}
for some $\alpha_t' \in [0, \alpha_t\beta^{-1}]$. Taking the limit as $k\to \infty$, we have that $\alpha_t'\to 0$ and $\mathbb{D}([X_t + \alpha_t' d_t]_+)[d_t] \to \mathcal{G}(X')$, which implies 
$$
-\langle \mathcal{G}(X'), d' \rangle \leq -\sigma \langle \mathcal{G}(X'), d' \rangle, \:\: \text{i.e. } -(1-\sigma)\langle \mathcal{G}(X'), d' \rangle \leq 0
$$
Since $\sigma < 1$, it follows that 
$$
-\langle \mathcal{G}(X'), d' \rangle = ||\mathcal{G}(X')||_F^2 \leq 0
$$
which contradicts the non-stationarity of $X'$. Hence, the limit point $\hat{X}$ is a stationary point. \qedsymbol

\subsection{Sequential Quadratic Programming (SQP)}

Taking the Newton direction as the descent direction can speed up the convergence to a stationary point.



\subsection{Sequential Subspace Method (SSM)}
\label{sec:sqp}
Here we introduce an efficient iterative method capable of global convergence to high-quality stationary points. We apply this method to refine the approximate solutions produced using the method introduces in Section \ref{sec:approx}. Motivated by the similarity between \eqref{eq:rescaled_f} and standard trust-region subproblems, we apply the framework of SSM. In the $k=1$ and $C=I$ case, SSM has been applied to Trust-Region sub-problems with remarkable empirical results~\cite{Hager2001MinimizingAQ} and robust global convergence guarantees~\cite{Hager2005GlobalSSM}, even for so-called degenerate problems. At a high level, SSM-based algorithms generate a sequence of iterates $X_t$ by solving a series of rescaled quadratic programs (of the same form as \eqref{eq:rescaled_f}) in subspaces of dimension much smaller than that of the original problem.  

At step $t$, we introduce a subspace $S_t$ derived from the current iterate $X_t$, the gradient of the objective of Prob. \eqref{eq:rescaled_f} $g_t=LX_tC - BC^{1/2}$, an \emph{SQP} (i.e. Newton's method applied
to the first-order optimality system $X_t$) iterate $X_{\text{sqp}}$ derived in Prop.~\ref{prop:newton}, and the principal eigenvectors of $L$. The Sequential Quadratic Programming (SQP) framework~\cite{nocedal99sqp} is applied to compute $X_{\text{sqp}}$.

Following the principle of SQP, we introduce the SQP direction $Z$ according to the linearization of \eqref{eq:rescaled_f_foc}, the first-order conditions of \eqref{eq:rescaled_f}:
\begin{align*}
(LZC - Z\Lambda) - X \Delta = E &:= BC^{1/2} - (LXC - X\Lambda), \quad
X^\top Z = 0
\end{align*}
%
\begin{proposition}[SQP iterate of the Lagrangian of \eqref{eq:rescaled_f_lagrangian}]
Assume $\Lambda$ is symmetric. Let $P^\perp = I - X^\top X$ be the projection onto the orthogonal complement of the column space of $X$ and $\Lambda C^{-1} = U\text{diag}([\lambda_1,\ldots,\lambda_k]) U^{-1}$ be the eigenvector decomposition of $\Lambda C^{-1}$. The Newton direction $Z$ of $X$ via the linearization of the first-order conditions is 
%
\begin{equation}
  Z = OU^\top,
  \label{eq:sqp}
\end{equation}
%
where each column of $O$, $o_j = (P^\perp LP^\perp - \lambda_j P^\perp)^\dagger BC^{-1}u_j$.
\label{prop:newton}
\end{proposition}
%
\emph{Proof.} Recall the FOC and its associated linearization with respect to descent directions of $X, \Lambda$; $(Z, \Delta)$:
\begin{align*}
&(LZC - Z\Lambda) - X \Delta = E := BC^{1/2} - (LXC - X\Lambda) \\
&X^\top Z = 0
\end{align*}
Applying the projection $P^{\perp} = I - XX^\top$ eliminates the $X\Delta$ term:
$$
PLZ - Z\Lambda C^{-1} = PLPZ - ZU\text{diag}([\lambda_1, \ldots, \lambda_k])U^{-1} = PEC^{-1}
$$
Equivalently, 
$$
PLPZU - ZU\text{diag}([\lambda_1, \ldots, \lambda_k]) = PEC^{-1}U.
$$ 
Let $O = ZU = [o_1,\ldots, o_k]$ lie in the range of $P$. Then, 
$$
PLo_j - \lambda_j = PEC^{-1}u_j, \text{ so } o_j = (PLP - \lambda_j P)^\dagger EC^{-1}u_j.
$$ \qedsymbol
%
\begin{algorithm}
\caption{SQP Update}
\begin{flushleft}
\textbf{Input:} Partial Laplacian $L$, affine term $B$, intermediate feasible iterate $X_t$, scaling term $C$\\
\textbf{Output:} $j-th$ columns of Newton updates\textemdash $\Delta_j, Z_j$
\end{flushleft}
\begin{algorithmic}[1]
\Function{SQP}{$L, \Lambda_t, B, X_t$}
\State $\Lambda_t = X_t^\top (LX_t C - BC^{1/2})$
\State $U\text{diag}([\lambda_1, \ldots \lambda_k])U = \Lambda C^{-1} = C^{-1/2}\Lambda_t C^{-1/2}$ 
\State init $O$, $P^\perp = I - X^\top X$
\For{$j \in [k]$}
    \State $o_j = (P^\perp L P^{\perp})^{\dagger}BC^{-1}u_j$
\EndFor
\State \Return $OU^\top$
\EndFunction
\end{algorithmic}
\label{alg:sqp}
\end{algorithm}
%
\noindent Alg.~\ref{alg:sqp} presents the detailed steps involved in the computation of the Newton directions, i.e. Prop.~\ref{prop:newton}. In Section~\ref{sec:complexity}, we discuss its computational cost.

\textbf{Computation of the SQP iterate}
Note that $\lambda_j$ appears in the computation of the pseudo inverse of $P^\perp L P^\perp - \lambda_j P^\perp$. To ensure that $P^\perp L P^\perp - \lambda_j P^\perp$ is positive semi-definite, we introduce a \emph{safeguard} to adjust $\lambda_j$ manually. 
%
\begin{proposition}[Safeguard for $\lambda_j$]
$\lambda_j$ are chosen to be the eigenvalues of $\Lambda C^{-1}$. Let
$$
P_1^{\perp} = P^{\perp} + x
$$
\end{proposition}
We note that the safeugarding $\lambda_j$ introduces additional computational  our algorithm. In practice, we observe that safeugarding is not necessary\textemdash i.e. for all of our experiments, we forgo safeguarding to save computation. 

Although stationary points can be recovered via an iterative project-descent procedure using gradient-based or SQP-based descent directions, we introduce the Sequential Subspace Method (SSM) in Alg.~\ref{alg:ssm}: a computationally friendly algorithm to address scalability with respect to large problems. Our development of SSM is inspired by the $1$-dimensional algorithm of \cite{Hager2001MinimizingAQ}, originally proposed to solve large trust-region subproblems. In other words, instead of solving \eqref{eq:cneqi} directly as previously mentioned, we instead solve a sequence of quadratic programs in subspaces of much smaller dimension relative to the size of the graph (the dimensions of $L$). SSM generically involves repeating the following pair of steps:
%
\begin{enumerate}
    \item Compute the SQP direction $Z = \text{SQP}(L,\Lambda, B, X)$ as defined in Prop.~\ref{eq:sqp} and Alg.\ref{alg:sqp}, line 5.  Let $V$ be the orthogonal matrix consisting of columns in $S$ (Alg.\ref{alg:ssm}, lines 6 and 7), where
    $$
    S = \text{span}(X_t, Z_t, u, g_t).
    $$
    \item SSM generates an approximation of $(X,\Lambda)$ and an approximation of the smallest pair of eigenvalues $\sigma$ and eigenvectors $u$ of $L$ in the subspace $S$,
    $$
    [X,\Lambda, u, \sigma] = \text{SSM}(L, B, S)
    $$
    consider the approximation $X = V \widetilde{X}$ for some $\widetilde{X}$. Compute
    \begin{equation}
    \min_{\widetilde{X} \in \text{St}(\widetilde{n},k)}F_{S} := \min_{\widetilde{X}}F(\widetilde{X}; V^\top L V, V^\top B).
    \label{eq:subspace_prob}
    \end{equation}
    %We can consider $v = V\tilde{v}$ to be a matrix consisting of estimates of the eigenvectors of $L$, if $\tilde{v}$ corresponds to a pair of eigenvectors of $B$ associated with its smallest two nontrivial eigenvalues (Alg.\ref{alg:sqp}, line 9).
\end{enumerate}
%
Note that \eqref{eq:subspace_prob} is solved using the Projected Gradient Method, where the projection is given by \cref{rem:stiefel_projection}: $[X]_+ = UV^\top$. %, where $U$ and $V$ are given by the singular value decomposition; $U\Sigma V^\top = \text{SVD}(X)$. 
We update $\Lambda$ according to the least-squares estimate derived from the first order condition in \eqref{eq:rescaled_f_foc} $\Lambda = X^\top (AXC - BC^{1/2})$.

We highlight that the sequence of iterates generated by SSM exhibits the following global convergence property, which we discuss further in the appendix.

%\input{statements/ssm_convergence.tex}
\ssm*

%
\begin{algorithm}
\caption{Sequential Subspace Minimization}
\begin{flushleft}
\textbf{Input:} Partial Laplacian matrix $L$, unit vector $u$\\
\textbf{Output:} Embedding coordinates $X$
\end{flushleft}
\begin{algorithmic}[1]
\Function{SSM}{$A, u$}
\State $L \gets D - A$ \Comment{Compute the graph Laplacian}
\State Initialize $X$ according to Sec~\ref{sec:approx}.
\While{not converged} 
\State $Z \gets SQP(L, \Lambda, B, X, u)$ \Comment{Eq.~\ref{eq:sqp} \& Alg. 2}
\State $\mathcal{S} \gets \text{span}(X_t, Z_t, u, g_t)$
\State $V \gets QR(\text{col}(S))$
\State $\widetilde{L} \gets V^\top L V$, $\widetilde{B} \gets V^\top B$
%\State $X \to \min_X F(X; B, V^\top B)$ \Comment{Solve \eqref{eq:sqpobj} in $S$}
%\State $\tilde{X} \to \min_{X\in St(dim(V),k)} F(X; \tilde{L}, \tilde{B})$ \Comment{Solve Eq.~\ref{eq:rescaled_f} in $S$}
\State $\widetilde{X} \gets \min_{X:X^\top X = I} F(X; \widetilde{L}, \widetilde{B})$ \Comment{Solve Eq.~\ref{eq:rescaled_f} in $S$}

\State $X_t \gets V^\top \widetilde{X}$ \Comment{Lifted coordinates}
\State $t \gets t+1$
\EndWhile
\State \Return $X_t$ 
\EndFunction
\end{algorithmic}
\label{alg:ssm}
\end{algorithm}
%
\subsection{Convergence of SSM}

The proof follows from the associated result for the Projected Gradient Method, Prop.~\ref{prop:pgd_convergence}\textemdash i.e. applying the Projected Gradient Method with step sizes chosen according to the Armijo rule ensures that any limit point $X_*$ is a stationary point, when $d_t = -(LX_tC - BC^{1/2}) \in S_t$. Let $V_t$ be an isometry, consisting of vectors in $S_t$ computed via a QR-factorization. Let $L_t := V^\top_t L V_t$ and $B_t = V_t^\top B$. Then, $F(\widetilde{X}; L_t, B_t)$ be the corresponding objective in $S_t$. SSM computes $X_{t+1} = V_t\widetilde{X}$, where
$$
\widetilde{X} := \argmin_{\widetilde{X}} F(\widetilde{X}; L_t, B_t)
$$
Note that the sequence $\{X_1,\ldots, X_t, \ldots\}$, with $X_{t+1}\in V_t$ monotonically reduces $F$ with respect to $t$:
\begin{flalign*}
F(\widetilde{X}; L_t, B_t) &= \frac{1}{2}\langle X_{t+1}, LX_{t+1}C - 2BC^{1/2} \rangle \\
&\leq \min_{\widetilde{X}}\{\frac{1}{2}\langle V_t\widetilde{X}, LV_t\widetilde{X}C - 2BC^{1/2} \rangle = \frac{1}{2}\langle \widetilde{X}, L_t\widetilde{X}C - 2B_tC^{1/2} \rangle = F(\widetilde{X}; L_t, B_tC^{1/2})\} \\
&\leq \frac{1}{2}\langle X_t, LX_tC - 2BC^{1/2} \rangle = F(X_t; L, B)
\end{flalign*}
For each $t$, since the columns of $X_t$ and $LX_tC - BC^{1/2}$ lie in $S_t$, the iterations of the gradient projection method with Armijo rule lie in $S_t$, and the sequence with decreasing objective reaches a stationary point $\widetilde{X}$, it is ensured that the first order condition
$$
AX_*C - BC^{1/2} = X_*\Lambda_*
$$
holds for some matrix $\Lambda_* \in \mathbb{R}^{k\times k}$, given by
$$
\Lambda_* = X_*^\top (LX_*C - BC^{1/2}) = \lim_t X_t^\top(LX_kC - BC^{1/2})
$$
In the case $C = I$, the following states that the inclusion of $[v_1, \ldots, v_k]$ in $S_t$ improves the quality of the stationary point $X_*$, characterized by the eigenvalues of $\Lambda$.

\begin{proposition}[Convergence of SSM]\label{prop:ssm_convergence}
Assume $C = I$. Let $X_* := [x_1,\ldots,x_k]$ be a stationary point generated from SSM. Then,
$$
LX_* - X_*\Lambda_* = B.
$$
Let $\lambda_1,\ldots,\lambda_k$ be the eigenvalues of $\Lambda_*$ and let the eigenvalues of $L$ be $d_1 \leq d_2 \leq \ldots \leq d_n$. Then, $\max\{\lambda_1,\ldots,\lambda_k\} \leq d_k$. 
\end{proposition}

\emph{Proof. } Let $X_t = [x_{1,t}, \ldots, x_{k,t}]$ be a global minimizer in $V_{t-1}$. let $Y_t := [y_{1,t}, \ldots, y_{k,t}] = V_{t-1}^\top [x_{1, t}, \ldots, x_{k,t}]$. Then,
$$
L_{t-1}Y_t - B_{t-1} = Y_t \Lambda_t
$$
holds for some $\Lambda_k$ with eigenvalues $[\lambda_{1,t}, \ldots, \lambda_{k,t}]$. In addition, since $Y_tB_{t-1} = X_tB$, then $X_tB$ is positive semidefinite and symmetric. As $t \to \infty$, $X_*^\top B$ is also positive semidefinite and symmetric. Additionally, let
$$
P_j^{\perp, (t)} = I - \sum_{i \in \mathcal{R} - {j}} y_{i,t}y_{i,t}^\top.
$$
The second order condition implies
$$
P_j^{\perp, (t)}LP_j^{\perp, (t)} - \lambda_{j,t}P_j^{\perp, (t)} \succeq	0.
$$
Consider the optimality of $x_{1,t}$. Let $\phi_{1,t}$ by a unit vector orthogonal to $[x_{2,t},\ldots, x_{k,t}]$ in $span\{v_1,\ldots,v_k\}$. Then $P_j^{\perp, (t)}V_{t-1}^\top \phi_{1,t} = V_{t-1}^\top\phi_{1,t}$ holds and the second order condition yields
\begin{flalign*}
0&\leq \langle V_{t-1}^\top\phi_{1,t}, (P_j^{\perp, (t)}LP_{j,t}^{\perp} - \lambda_{j,t}P_{j,t}^{\perp})V_{t-1}^\top \phi_{1,t} \rangle \\
&= \langle \phi_{1,t}, (L - \lambda_{1,t}I)\phi_{1,t}\rangle\\
&\leq (\min_i d_i - \lambda_{1,t})||\phi_{1,t}||^2,
\end{flalign*}
Which implies $\lambda_{1,t} \leq \min_i d_i$. As $t \to \infty$, a subsequence of $\{x_{1,t}, \ldots, x_{k,t} : t \}$ converges to $[x_1,\ldots, x_k]\in \mathcal{M}$ and $\lambda_{1,t}$ converges to $\lambda_1$ Hence, $\lambda_1 \leq \min_i d_i$. Likewise, $\lambda_j \leq \min_i d_i$ by the optimality of $x_{j,t}$ for $j = 2,\ldots, k$. \qedsymbol

The following is the result of \Cref{prop:ssm_convergence}.
%\input{statements/ssm_convergence.tex}
\ssm*

\textbf{On convergence to globally optimal solutions}

We briefly and informally discuss the necessary conditions for \emph{global optimality} of \eqref{eq:rescaled_f}, under the assumption that $C= I$. For simplicity, take $k=2$. And denot $\lambda_1, \lambda_2$ the eigenvalues of $\Lambda$. We can prove that for any local minimizer $X$, if the associated eigenvalues $\lambda_1,\lambda_2$ are both less than $d_1$, the smallest nonzero eigenvalue of $L$, that $X$ is a global minimizer. As we have shown, with proper initialization, our method recovers a local minimizer $X$ such that $\lambda_1, \lambda_2$ are both less than $d_2$. There are several potential avenues to prove that any local minimizer is also a global minimizer. For example we could impose an eigenvector-preserving transformation to $L$ or restrict our analysis to graphs such that $\lambda_i = \lambda_k$ where $\lambda_i \geq 0$. 

An alternative method is to ensure a non-degenerate condition on $B$ as in canonical trust-region methods. Briefly, let $v_1, \ldots, v_k$ be the eigenvectors of $L$ corresponding to $k$ smallest nonzero eigenvalues $d_1 \leq \ldots \leq d_k$. At a high level, we need to ensure that the columns of $B$ are not nearly orthogonal to $v_1, \ldots, v_r$

\begin{proposition}
Let $V = [v_1, v_2]\in \mathbb{R}^{n \times 2}$ be the eigenvectors of $L$ corresponding to the smallest two nonzero eigenvalues $d_1 \leq d_2$. Let $X$ be a local solution satisfying the first order condition 
$$
AX = X\Lambda + B
$$
and second order condition $\lambda_1, \lambda_2 \leq d_2$. Let $s_1$ be the smallest singular value of $V^\top B$. Suppose
$$
s_1 > d_2 - d_1
$$
Then, the eigenvalues $\lambda_1, \lambda_2$ of the Lagrangian multipliers $\Lambda$ are less than $d_1$ and $X$ is a global minimizer.
\end{proposition}
\emph{Proof. } Recall that the second order condition is 
$$
\lambda_j \leq d_2 \text{ for } j = 1,2.
$$
Consider the first order condition $LX = X\Lambda + B$. Taking an inner product with $v_2$ and $v_1$ yields
\begin{flalign*}
&d_2 v_2^\top X = v_2^\top LX = (v_2^\top X)\Lambda + v_2^\top B, \\
&d_1 v_1^\top X = v_1^\top LX = (v_1^\top X)\Lambda + v_1^\top B.
\end{flalign*}
Let $u_1$ and $u_2$ be eigenvectors of $\Lambda$ associated with eigenvalues $\lambda_1, \lambda_2$. For $j=1,2$, taking the product with $u_j$ on the r.h.s yields
$$
(d_2 - \lambda_j)v_2^\top Xu_j = v_2^\top Bu_j,\:\: (d_1 - \lambda_j)v_1^\top Xu_j = v_1^\top Bu_j 
$$
Since $||V|| = 1 = ||X||$, then $||V^\top X u_j||\leq ||Xu_j|| \leq 1$. Thus,
$$
|d_2 - d_1| < s_1 \leq ||V^\top B u_j|| \leq \min(|d_2 - \lambda_j|,|d_1 - \lambda_j|)||V^\top X u_j|| \leq \min(|d_2 - \lambda_j|,|d_1 - \lambda_j|)
$$
which implies $\lambda_j < d_1$.

\label{sec:complexity}
\subsection{Complexity of SSM}
In this section, we discuss the computational cost of our method, dominated by the SQP routine
to compute the SQP directions. We claim that the per-iteration complexity of our algorithm is $T_{\text{matrix}}$, where $T_{\text{matrix}}$ is the complexity of each call to a sparse matrix (i.e. Laplacian, more generally an \emph{M-matrix}) solver. In particular, the QR-decomposition of $\text{col}(S)$ takes time linear in $n$. Likewise, fast, nearly linear-time solvers exist for solving Laplacian and Laplacian-like systems that are robust to ill-conditioning~\cite{spielmanteng}. We adopt Multigrid preconditioned conjugate gradient due to its empirical performance. We further note that the SSM procedure itself exhibits quadratic rates of convergence for nondegenerate problems and global convergence with \emph{at least} linear rates, even when the problem exhibits certain degenerate characteristics~\cite{Hager2005GlobalSSM}. 

%Generic quadratic programs are NP-hard~\cite{Pardalos1991QuadraticPW}, i.e. it takes super-polynomial time to solve QPs optimally. In the convex case, there are polynomial time interior point algorithms~\cite{dikininteriorpoint}. Also, there are approximation algorithms that return local solutions of nonconvex QPs in polynomial time~\cite{Hager2001MinimizingAQ}. Our method falls into the category of algorithms that guarantee local, or block-globally optimal solutions.

%In particular, although the objective of our algorithm satisfies the conditions for convexity, the addition of quadratic equality constraints introduces a violation of the conditions necessary for convexity.

\subsubsection{Computation of the descent direction $Z$}

In Sec 3.3, we express the SQP direction $Z$ as the solution to the system characterized by the linearization of the first order optimality conditions. Namely, within each iteration of our procedure, we compute the Lagrangian multipliers as well as the SQP update for $X$ as defined in \eqref{eq:sqp}. As in Newton's method for unconstrained problems, SQP-based methods necessitate computation of inverse-vector products involving symmetric PSD matrices. 

We assume that by exploiting the sparsity of $L$, vector-vector and matrix-matrix multiplication can be done in linear time. In Alg.~\ref{alg:sqp}, we present the the SQP routine. The computation in line 3 involves an eigenvalue decomposition of a small $k\times k$ matrix. Thus, the primary overhead of our method lies in the computation of each column of $O$; $o_j, j = 1,\ldots, k$, which necessitates computation of $k$ Laplacian-like pseudoinverse-vector products. 

\iffalse
To compute the inverses in line 7, we first compute $L_{W_j}^{-1}E$ by solving the linear system $L_{W_j}b = E$ for $b$. We solve ${X^\top L_{W_j}^{-1}X}\delta_j = b$ for $\delta_j$. Using conjugate gradient, with an appropriate preconditioner $K$, the computation of $\delta_j$ up to a residual $\epsilon$ can be done in $O(n\sqrt{\kappa(KL)}\log(1/\epsilon))$ time. The computation of $Z_j$ can be done in the same way.

In other words, the computation of the columns of the Lagrangian multipliers $(\Delta)_j$ can be decomposed into (1.) the computation of $L+W_jI$ twice in $O(n)$ time (2.) its inverse three times (once for each column of $X$ and once for $E_j$) via conjugate gradient, again in $O(n\sqrt{\kappa(KL)}\log(1/\epsilon))$ time (3.) two left-multiplications by $X^\top$ in $O(2n)$ time. To compute the columns of the Newton direction; $Z_j$, first note that $P$ can be rewritten as $I-vv^\top$. Then, $(W_jI)^{-1} P = (W_jI)^{-1} - ((W_jI)^{-1}v)v^\top$.
\fi

%In summary, the complexity of our method is dominated by the computation of the SQP newton direction $Z$ in line 5 of Alg.~\ref{alg:ssm}, due to the necessity of computing $k$ unique inverse-vector products involving the Laplacian (lines 7 and 10 of Alg.~\ref{alg:sqp}).

%\chester{Explain SSL vs procrustes and discuss (SSL linear transforms orthogonal eigenvectors to match predictors - we fix the vectors and align eigenvectors of other matrix with labels).}
\iffalse
\subsection{Perturbation estimate for eigenvalues of $L_\mathcal{U}$}

If we have $L_\mathcal{U \setminus \{ \emph{i} \}} = L_\mathcal{U} + E^i$, then if $\lambda$ is an eigenvalue of $L_\mathcal{U}$, the corresponding eigenvalue of of $L_\mathcal{U} + E^i$ can be expressed as $\lambda^* = \lambda + \lambda' = \lambda + \delta \lambda^{(1)} + \delta^2 \lambda^{(2)} + \ldots$ where $\lambda^{(i)}$ are eigenvalues of other matrices. As we discussed earlier, Weyl's inequality and Gershgorin circle theorem could imply some lower-bounds. 

Consider a grounded Laplacian $L_\mathcal{U}$ and the associated perturbation implied by labeling a vertex $E^i = \sum_{j \in \mathcal{U}}A_{ij} (E_{ij} + E_{ji})$, where $E_{ij}$ is an $n\times n$ matrix with $1$ in the $ij$-th position (and, to be clear, $A_{ij}$ is a scalar). Let $u$ be one eigenvector of $L_\mathcal{U}$. Then, we have that:
%
$$
(L_\mathcal{U} + E^i)(u + u') = (\lambda + \lambda')(u + u')
$$
%
Multiply both sides by $u^\top$ and eliminate the common terms:
\begin{flalign*}
&\mathbf{u^\top L_\mathcal{U} u} + \mathbf{u^\top L_\mathcal{U} u'} + u^\top E^i u + u^\top E^i u' = \mathbf{u^\top \lambda u} + \mathbf{u^\top \lambda u'} + u^\top \lambda' u + u^\top \lambda' u' \\
&\implies u^\top E^i u + u^\top E^i u' = u^\top \lambda' u + u^\top \lambda' u' \\
&\implies u^\top E^i (u + u') = u^\top \lambda' (u + u') \\
&\implies 
\lambda' = \frac{u^\top E^i (u+u')}{1 + u^\top u'}  
\end{flalign*}
In the limit of unlabeled data, we have that $u' \to 0$. Then, $\lambda ' \to u^\top E^iu = 2u_i \sum_{j \in \mathcal{U}} A_{ij} u_j \approx \tilde2{d}_{ii}u_i^2$
\fi

\subsection{Cut-based refinement}
\label{sec:cutrefinement}
\begin{algorithm}
\caption{Kernighan-Lin refinement}
\begin{flushleft}
\textbf{Input:} KNN weights $W$\\
\textbf{Output:} Predictions $X$
\end{flushleft}
\begin{algorithmic}[1]
%\Function{KL}{$W$}
\State Compute $g(v)$ for all $v \in \mathcal{V}$ %$D_i = \sum_{j | \ell(v_i) = \ell(v_j)}W_{ij} - \sum_{j | \ell(v_i) \neq \ell(v_j)}W_{ij}$ for all $i \in V$ \\
\While{not converged} 
\For{each pair of $n\choose 2$ partitions (classes) $\mathcal{V} = (\mathcal{V}_1, \mathcal{V}_2)$}
\State ordered list $l \gets \emptyset$ 
\State unmark all vertices $v\in V$ 
\For{$i=1$ to $n=\min(|\mathcal{V}_1|, |\mathcal{V}_2|)$}
\State $(v_1, v_2) \gets \argmax_{v_1, v_2} g(v_1, v_2)$
\State update $g$-values for all $v \in N(v_1) \cup N(v_2)$
\State add $(v_1, v_2)$ to $l$ and mark $v_1, v_2$
\EndFor
\State $k^* \gets \argmax_k \sum_{i=1}^kg(v_i, w_i)$ 
\State Update $(\mathcal{V}_1, \mathcal{V}_2)$: swap $(v_i, w_i) \in l$, $i = 1,\ldots,k^*$
\EndFor
\EndWhile

%\EndFunction
\end{algorithmic}
\label{alg:kl}
\end{algorithm}

In this section, we provide a detailed overview of the Kernighan-Lin (KL) algorithm and our multi-class extension.

The Kernighan-Lin algorithm \cite{klin1970} iteratively improves a given a disjoint bipartition of $\mathcal{V}$: $(\mathcal{V}_1, \mathcal{V}_2)$ such that $\mathcal{V}_1 \cup \mathcal{V}_2 = \mathcal{V}$, by finding subsets of each partition $A \subset \mathcal{V}_1$, $B \subset \mathcal{V}_2$ and then moving the nodes in $A$ and $B$ to the  opposite block. More concretely, the Kernighan-Lin algorithm repeatedly finds candidate sets $A$, $B$ to be exchanged until it reaches a local optimum with respect to the cut objective. Notably, the algorithm has the desirable tendency to escape poor local minima to a certain extent due to the way in which the sets $A$ and $B$ are created. This is one of the key features of the algorithm, and is a critical advantage over gradient-based methods for partitioning refinement, such as the MBO method presented in \cite{calder20poisson}.

The gain of a vertex $v$ is defined $g(v) = \sum_{j | \ell(v_i) = \ell(v_j)}W_{ij} - \sum_{j | \ell(v_i) \neq \ell(v_j)}W_{ij}$. , i.e. the reduction in the cut cost when the vertex $v$ is moved from partition $V_1$ to partition $V_2$. Thus, when $g(v) > 0$ we can decrease the cut by $g(v)$ by moving $v$ to the opposite block. Let $g(v,w)$ denote the gain of exchanging $v$ and $w$ between $V_1$ and $V_2$. Analogously, if $v$ and $w$ are not adjacent, then the gain is $g(v, w) = g(v) + g(w)$. If $v$ and $w$ are adjacent, then $g(v, w) = g(v) + g(w) - 2\omega(v, w)$.

The KL algorithm characterizes each vertex in $G$ as having one of two states: marked or unmarked. At each pass of the algorithm, each node is unmarked. A KL pass proceeds by iteratively finding an unmarked pair $v \in \mathcal{V}_1$ and $w \in \mathcal{V}_2$ for which $g(v, w)$ is maximum (note that $g(v, w)$ is not necessarily positive), marking $v$ and $w$, and updating the gain values of each of remaining unmarked nodes (i.e. the neighbors of $v$ and $w$) assuming an exchange between $v$ and $w$. This procedure repeats $p= \min(|\mathcal{V}_1|, |\mathcal{V}_2|)$ times.

After $p$ iterations, we have an ordered list $l$ of vertex pairs $(v_i , w_i)$, $i = 1,\ldots , p$. The swap-sets $A$ and $B$ are derived by finding the smallest index $k \in \{0,\ldots , p\}$ such that $P = \sum^k_{i=1} g(v_i, w_i)$ is maximum. Then, $A := \bigcup^k_{i=1}\{v_i\}$ and $B := \bigcup^k_{i=1}\{w_i\}$. A nonzero $k$ implies a reduction of the cut cost if $A$ and $B$ are exchanged. In this case, the exchange is performed and a new pass is instantiated. Otherwise, the KL iterations conclude.

Note that KL is typically performed over bi-partitions. We extend this framework to $k$-partitions in Algorithm~\ref{alg:kl} by considering a randomly ordered set of $k \choose 2$ pairs of classes (as defined by the predictions made on the vertex set) and performing KL on the subgraph restricted to these vertices. This procedure continues iteratively until all $k\choose 2$ pairs have been exhausted. Then, if convergence or a predetermined number of iterations has not been reached, a new random sequence is generated and the procedure continues.

\section{Graph-Based Active Learning}
\label{sec:graphal}
In this section, we introduce an active-learning scheme motivated by the criticality of label selection at low label rates and the benefits of diversity sampling. 
%In particular, we are motivated by the low label-rate regime. 
In the low label-rate regime, it is well-known that active learning strategies which emphasize \emph{exploration} of the sample-space, i.e. \emph{diversity} of the labeled samples, outperform those that rely on \emph{exploitation} of a classifiers decision boundary, e.g. notions of margin \cite{miller2022poisson}. Therefore, we propose a computationally efficient technique inspired by algebraic methods for selecting landmarks in graphs\textemdash i.e. a method that aims to select well-connected vertices diversely over the graph (vertices with large degree that are maximally separated) according to the spectral properties of the Laplacian. %We discuss that when the graph is ill-specified or noisy, the quality of critical points is determined by the condition number of $L_\mathcal{U}$. 

\iffalse
\subsection{Active learning corresponds to additive perturbations of $L$}

Given a graph $G$ with adjacency matrix $A$ and Laplacian $L = D-A$, we may consider A under the following edge-perturbation noise model. Let the supplement of $A$ be given by $\bar{A} = 11^\top - I - A$. Let the boolean matrix $S \in \{0,1\}^{M\times M}$ encode whether an edge of $G$ is modified (added or removed) iff $S_{ij} = S_{ji} = 1$. The corresponding perturbation of $A$, $A'$ is then given by
$$
A' = A + \hat{A} \circ S,\quad \hat{A} = \bar{A} - A
$$
Thus, the corresponding perturbation to the Laplacian is given by $L' = L + ((\hat{A} \circ S)11^\top)\circ I - \hat{A} \circ S$

Recall that the FOC of our problem is the perturbed linear system
$$
(L + E_{L})X = (B + E_B) + X\Lambda 
$$
where $E_{L}$ and $E_B$ are two noise matrices. As we detail in the appendix, SSM guarantees convergence to certain high-quality critical points characterized by the eigenvalues of $\Lambda$ and $L$. These conditions imply a bound on the eigenvalues of $\Lambda$ (Prop. B.8). As a consequence, the $X\Lambda$ term of the FOC can be safely assumed to be negligeable at first-order optimal solutions (i.e. those produced by our algorithm). By additionally assuming $C=I$, the relative estimation error~\cite{GoluVanl96} of a linear system $(L + E_{L})X = (B + E_B)$ satisfies
\begin{flalign*}
\frac{||\hat{X} - X||}{||X||} &\leq \kappa(L)\left(\frac{||E_{L}||}{||L||} + \frac{||E_B||}{||B||}\right) 
\leq \epsilon \kappa(L) \left(\frac{1}{||L||} + \frac{1}{||B||}
\right)
\end{flalign*}
where $||\cdot||$ is an induced $\ell_2$ matrix norm, $\epsilon = \max (||E_{L}||, ||E_{B}||)$ the condition number of $L$, $\kappa(L) = \frac{\lambda_{\text{max}}}{\lambda_{\text{min}}}$. Assuming the relative magnitude of the noise is small, this motivates finding $\mathcal{U}$ such that $L = PL_\mathcal{U}P$ has good conditioning.
\fi

\subsection{Spectral score for diversity sampling on graphs}
\input{figures/plots}
We propose to select vertices from the set of unlabeled vertices according to the following measure:
\begin{equation}
\argmax_{v_i} \{s(v_i) := \tilde{d}_{i}u_i^2\}
\end{equation}
where $\tilde{d}_{i}$ denotes the degree of vertex $i$ defined on the sub-graph associated with the set of unlabeled vertices, $\mathcal{U}$ and $u_i$ corresponds to the $i$-th entry of $u$, the solution to the boundary-constrained eigenvalue problem:
\begin{equation}\label{eq:bv}
\left.\begin{aligned}
\mathcal{L} u_i &= \lambda u_i,&&\text{if }m+1 \leq i \leq M \\
u_i &=0,&&\text{if }1 \leq i \leq m \\
\end{aligned}\right\}.
\end{equation}
%
%\begin{equation}
%u = \argmin\{\frac{u^\top L u}{||u||^2}\:\: |\:\: \text{supp}(u) \subset %\mathcal{U},\:\: u \in \mathbb{R}^n\}
%\end{equation}
%By the min-max theorem, 
Note that $\text{supp}(u)$ is nothing but the entries of the eigenvector corresponding to the smallest eigenvalue of $L_\mathcal{U}$. Naturally, $u_i$ encodes various notions of centrality. Notably, \citet{cheng2019diffusiongeom} demonstrate an intimate connection between the solution $u$ in \eqref{eq:bv} for a normalized random walk Laplacian and the absorption time of a random walk / diffusion distance of vertex $i$ with respect to the boundary vertices $l$. More concretely, they prove that for solutions to boundary-constrained eigenvalue problems defined for certain Laplacians (e.g. absorbing random walk Laplacians), the diffusion distance from vertex $i$ to the boundary, $d_{l}(i)$ satisfies the following inequality:
$$
d_{l}(i) \log\left( \frac{1}{ |1 - \lambda_1|} \right) \geq \log \left( \frac{2|u(i)|}{||u||_{L^\infty}} \right)
$$
In other words, $d_l$ is \emph{highly correlated} with $|u|$. While \citet{cheng2019diffusiongeom} derive this relationship explicitly for $|u_i|$, we empirically show that selecting vertices for active learning in this way performs poorly relative to state of the art methods. Inspired by recent sampling strategies for graph signal reconstruction~\cite{ajinkya2018distancesampling} in the presence of noise, we demonstrate \emph{reweighting} $u_i^2$ by $\tilde{d}_i$ is an effective and principled heuristic. Additional details are provided in the supplemental material. Notably, we highlight that this score \emph{comes at no extra computational cost} due to certain features of SSM\textemdash in particular SMM's capability of producing estimates of the eigenvectors of $L$ in addition to solutions of \eqref{eq:rescaled_f}.

Intuitively, the proposed score naturally encodes the eigenvector centrality and degree of a vertex as well as its geodesic distance to labeled vertices. In practice, we incorporate eigenvectors of higher order eigenvalues as well as interpolate towards a margin-based score as the label-rate increases, setting the score to:
$$
s(v_i) = ||\tilde{d}_{i} \odot U_i^2||_2,
$$
where $U$ is now an $n\times \ell$ matrix with eigenvectors as columns and $U_i^2$ denotes the matrix consisting of the square of the elements of column $U_i$. The choice of $\ell$ is left as a hyperparameter. In our experiments, we use $\ell=3$.
%
\begin{remark}
If $\mathcal{U}^c$ corresponds to the empty set, it is apparent that the smallest eigenvalue of $L_\mathcal{U} = \mathcal{L}$ is $0$, and the corresponding eigenvector is $u=1$. Hence, the acquisition score of each vertex is nothing but a constant times its degree.
\end{remark}
%
While the work of \citet{cheng2019diffusiongeom} provides concrete motivation for our method, we derive the following property that ensures samples are diverse, i.e. far from the labeled nodes.
\iffalse
\begin{proposition}
Let $N_i$ denote the neighborhood of vertex $i$. Consider score at vertex $v_a$, $s(v_a) = |u_i|$. For any connected pair of vertices $v_a$ and $v_b$ such that $v_a \not \in N_s$, $v_b \in N_s$ for any $s \in \mathcal{U}$, there is a path from $v_a$ to $v_b$ such that the sequence of entries $(s(v_a),\ldots, s(v_c), \ldots s(v_b))$ is nonincreasing.
\end{proposition} 
\fi
%%%%%%
the component of score involving the eigenvector of $L_\mathcal{U}$ associated with the smallest eigenvalue is motivated primarily by previous work that investigates features encoded by the eigenvectors of the Laplacian of a graph with grounded vertices~\cite{cheng2019diffusiongeom}. These features specifically facilitate efficient methods to diversely sample the graph. Additionally, our score has connections to the graph signal processing literature~\cite{ajinkya2018distancesampling,anis215graphsampling} which aims to robustly recover a graph signal by sampling a sparse set of vertices. It has been demonstrated that one ideal sampling strategy that is robust to noise aims to maximize the smallest eigenvalue of the principal submatrix of the Laplacian, analogous to $L_\mathcal{U}$. Below, we demonstrate that our method, namely squaring the entries of $u$ and weighting by $\tilde{d}_i$, is directly related to one lower bound of the smallest eigenvalue of $L_\mathcal{U}$.

\subsubsection{Lower bound estimate for eigenvalues of $L_\mathcal{U}$}
Consider a grounded Laplacian $L_\mathcal{U}$ and the associated perturbation implied by labeling a vertex $E^i = \sum_{j \in \mathcal{U}}A_{ij} (E_{ij} + E_{ji})$, where $E_{ij}$ is an $n\times n$ matrix with $(L_\mathcal{U})_{ij}$ in the $ij$-th position (and, to be clear, $A_{ij}$ is a scalar). Let $u$ be one eigenvector of $L_\mathcal{U}$. Then, we have that the bound essentially follows from a proof of Weyl's inequality~\cite{horn13}.  If $G$ is connected or $|\mathcal{U}^c| > 0$, the eigenvectors of $L_\mathcal{U}$ form a basis for $\mathbb{R}^n$.
Let $v$ be a unit eigenvector of $L_\mathcal{U} - E^i$ with eigenvector decomposition (where $u^{(j)}$ is the eigenvector associated with the $j$-th eigenvalue of $L_\mathcal{U}$ ).
$$
v = \sum_{j=1}^n t_j u^{(j)}
$$
for some coefficients $t_j$ s.t. $\sum_j t_j^2 = 1$. Then the eigenvalue $\lambda '$ of $L_\mathcal{U} - E^i$ is
\begin{equation}
\lambda' = v^\top (L_\mathcal{U} - E^i)v = \sum_{j=1}^n t_j^2 (\lambda_j - \langle u^{(j)}, E^i u^{(j)} \rangle) \geq \min_{j=1,\ldots,n}\{\lambda_j - \langle u^{(j)}, E^i u^{(j)} \rangle\}
\end{equation}
Thus, the maximum perturbation of the smallest eigenvalue of $L_\mathcal{U} - E^i$ is bounded below by the largest eigenvalue of $E^i$ (recall that $E^i$ has nonzero entries associated with the $i$-th column and $i$-th row of $L_\mathcal{U}$). Hence, to increase the eigenvalue of $L_\mathcal{U}$, a greedy selection implies the choice of $i$ that maximizes $-\langle u^{(j)}, E^i u^{(j)} \rangle= 2u^{(j)}_i \sum_{k \in \mathcal{U}} A_{ij} u^{(j)}_k$.

Note that when the spectral gap of $L_\mathcal{U}$ is large, $j$ need not be taken over $[n]$. More concretely, suppose $\lambda_{k' + 1} - \lambda_1 > \epsilon$, where $\epsilon$ is the largest eigenvalue of $\{E^i\:\: : \:\: i=1,\ldots, n\}$. Note that $\lambda' \geq \lambda$. Then,
\begin{equation}
\lambda' \geq \min \{\min_{j=1,\ldots,k'} \{ \lambda_j -  \langle u^{(j)}, E^i u^{(j)} \rangle \}, \lambda_{k' + 1} - \epsilon\} \geq \min_{j=1,\ldots,k'} \{\lambda_j - \langle u^{(j)}, E^i u^{(j)} \rangle\}
\end{equation}
We highlight that the spectral gap of graph Laplacians of graphs constructed on data, particularly KNN graphs, exhibit fast growth of the eigenvalues~\cite{ulriketutorial2007, lafondatafusion2006} and large spectral gaps. On such graphs, the low-frequency eigenvectors (eigenvectors corresponding to the smallest eigenvalues of the Laplacian) are ``smooth'' over the graph and the score presented in the main text is a good proxy for the above bound, i.e.
$2u^{(j)}_i \sum_{k \in \mathcal{U}} A_{ij} u^{(j)}_k \approx 2\tilde{d}_{i}(u_i)^2$. As we show below, using the ranking implied by \emph{just} $u_i$ corresponds to a diversity selection strategy that iteratively selects vertices that are far from the set of labeled nodes. Intuitively, weighting this measure by $\tilde{d}_i$ encourages selection of vertices that are \emph{well connected}. Experimentally, as shown in the main text, this also has the effect of improving results.

%
\iffalse
\begin{proposition}[Entries of the smallest eigenvector]
%For simplicity, let $\mathcal{L}$ be a normalized laplacian. Then, the eigenvalues of $\mathcal{L}$ are bounded between $-1$ and $1$. 
Let $u$ be the eigenvector of $L_\mathcal{U}$ corresponding to its smallest eigenvalue. For each vertex $v_i \in \mathcal{V} \setminus \mathcal{U}$, let $a_{v_i} = \frac{\sum_{v_j \in \{N_i \setminus u\}}u_j}{|\{N_i \setminus \mathcal{U}\}|}$. For any vertex $v_a$ such that $v_a \not \in N_s$ for any $s \in \mathcal{U}$ and $v_b$ such that $v_b \in N_s$ for some $s \in \mathcal{U}$, $a_{v_a} \geq u_i$ and $a_{v_b} \leq u_i$.
\end{proposition}

We have that the $ith$ entry of the eigenvectors of $L_\mathcal{U}$ are characterized by the system 
$$
d_i u_i - \sum_{v_j \in N_j \setminus \mathcal{U}}A_{ij}u_j = \lambda u_i.
$$
Note that
\begin{align}
\frac{\sum_{v_j \in \{N_i \setminus \mathcal{U}\}}u_j}{d_i} < u_i &= \frac{\sum_{v_j \in \{N_i \setminus \mathcal{U}\}}u_j}{d_i - \lambda }  \leq \frac{\sum_{v_j \in \{N_i \setminus \mathcal{U}\}}u_j}{d_i - 1}
\end{align}

Since the left-hand-side of the inequality corresponds to $a_{v_a}$ and right-hand-side corresponds to $a_{v_b}$, we have the bound.
\fi

\subsection{Spectral active learning score}
For the purposes of this section, we will consider a slightly different scoring function than the one presented in the main text. Let $s(v_i) = |u_i|$, where $u_i$ is the $i$-th component of the eigenvector of $L_\mathcal{U}$ corresponding to the smallest eigenvalue of $L_\mathcal{U}$. Note that 
%(1.) $0 < \lambda \leq 1$ due to interlacing and (2.) 
when the graph is connected, from the Perron-Frobenius theorem~\cite{1miekkalagraphprop93, horn13}, the eigenvector associated with the smallest eigenvalue of $L_\mathcal{U}$ can be chosen to be elementwise nonnegative.
\begin{proposition}
Let $N_i$ denote the neighborhood of vertex $i$. Consider the score at vertex $v_a$, $s(v_a) = |u_i|$. For any connected pair of vertices $v_a$ and $v_b$ such that $v_a \not \in N_k$, $v_b \in N_k$ for any $k \in \mathcal{U}^c$, there is a path from $v_a$ to $v_b$ such that the sequence of entries $(s(v_a),\ldots, s(v_c), \ldots s(v_b))$ is nonincreasing.
\end{proposition} 
\noindent \emph{Proof.} We will consider a vertex $v_i$ and its score $s(v_i)$ when its neighborhood does not contain a labeled vertex and its score $s'(v_i)$ when its neighborhood does contain a labeled vertex, $v_\ell$. First, note that the $ith$ entry of the eigenvectors of $L_\mathcal{U}$ are characterized by the system 
$$
d_i u_i - \sum_{v_j \in \mathcal{U}}A_{ij}u_j = \lambda u_i.
$$
Then, write $u_i = \frac{\sum_{v_j \in \mathcal{U}}A_{ij}u_j}{d_i - \lambda }$ and consider labeleing a single neighbor $v_\ell$ in the neighborhood of $v_i$:
%\begin{align}
%\frac{\sum_{v_j \in \{N_i \setminus \mathcal{U}\}}u_j}{d_i} < u_i &= \frac{\sum_{v_j \in \{N_i \setminus \mathcal{U}\}}u_j}{d_i - \lambda }  \leq \frac{\sum_{v_j \in \{N_i \setminus \mathcal{U}\}}u_j}{d_i - 1}
%\end{align}
%\begin{align}
%s(v_i) = \tilde{d_i}|u_i| = d_i\left| \frac{\sum_{j \in \mathcal{U}}A_{ij}u_j}{d_i - \lambda} \right|  &=  d_i\frac{\sum_{j \in \mathcal{U}}A_{ij}|u_j|}{|d_i - \lambda|} \\
%&\geq  d_i\frac{\sum_{j \in \mathcal{U}}A_{ij}|u_j|- |u_\ell|}{|d_i - \lambda|} = d_i\left | \frac{\sum_{j \in \mathcal{U}\setminus \{u_\ell\}}A_{ij}u_j}{d_i - \lambda} \right|\\
%&\geq (d_i-1)\left| \frac{\sum_{j \in \mathcal{U}\setminus \{u_\ell\}}A_{ij}u_j}{d_i - \lambda} \right| = s'(v_i)
%\end{align}
\begin{align}
s(v_i) = |u_i| = \left| \frac{\sum_{j \in \mathcal{U}}A_{ij}u_j}{d_i - \lambda} \right|  &=  \frac{\sum_{j \in \mathcal{U}}A_{ij}|u_j|}{|d_i - \lambda|} \\
&\geq  \frac{\sum_{j \in \mathcal{U}}A_{ij}|u_j|- |u_\ell|}{|d_i - \lambda|} = \left | \frac{\sum_{j \in \mathcal{U}\setminus \{u_\ell\}}A_{ij}u_j}{d_i - \lambda} \right|\\
& = s'(v_i)
\end{align}
Naturally, the implication is that the score of a vertex decreases as its neighbors are labeled. Furthermore we have that
%\begin{align}
%s(v_i) = \tilde{d_i}|u_i| &= \tilde{d_i}\left| \frac{\sum_{j \in \mathcal{U}}A_{ij}u_j}{d_i - \lambda} \right| \geq \frac{1}{d_i}|\sum_{j \in \mathcal{U}}\tilde{d_j}A_{ij}u_j| = \frac{1}{d_i}\sum_{j\in \mathcal{U}}A_{ij}s(v_j)
%\end{align}
\begin{align}
s(v_i) = |u_i| &= \left| \frac{\sum_{j \in \mathcal{U}}A_{ij}u_j}{d_i - \lambda} \right| \geq \frac{1}{d_i}\left|\sum_{j \in \mathcal{U}}A_{ij}u_j\right| = \frac{1}{d_i}\sum_{j\in \mathcal{U}}A_{ij}s(v_j)
\end{align}
Thus, the score of a vertex $v_i$ is greater than the average score of its neighbors, and therefore, there must be a neighbor of $v_i$ with score less than $s(v_i)$. 
%Note that the bound may not hold unless $|\mathcal{N}(v_i)|\tilde{d_i} \geq \sum_{j\in \mathcal{U}}\tilde{d}_j$
%
Since each vertex has a neighbor with smaller score, starting from any vertex there is a path consisting of vertices that have decreasing scores that must finish at a vertex with neighbor in $\mathcal{U}^c$. \hfill \qedsymbol

Again, we emphasize that this is not necessarily true when $|u_i|$ is weighted by the degree $\tilde{d_i}$. Including this weight is intuitively motivated by the principle of connectnedness. In other words, our score selects vertices \emph{that are both distant from the set of labeled vertices, \textbf{and} well-connected}.
%%%%%%
%
We provide an intuitive visualization of this score in Figure~\ref{fig:visualization}. The dataset is comprised of eight Gaussian clusters, each of equivalent size ($300$ samples), whose centers (i.e., means) lie evenly spaced apart on the unit circle. 
Each cluster is created by randomly sampling $300$ points from a Gaussian with mean $µ_i = (\cos(\pi i/4),\sin(\pi i/4))^\top\in \mathbb{R}^2$ and standard deviation $\sigma_i = \sigma = 0.17$. 
The class structure is then assigned in an alternating fashion. 
%In each individual run of the experiment, one initially labeled point per class combine to be the starting labeled set, and then $100$ active learning query points are selected sequentially via the lower-bound derived in equation~\ref{eq:activelearning}. 
For this example, efficient exploration via active learning is critical, particularly at low label rates. As we show in Figure~\ref{fig:visualization} our score facilitates effective exploration of the geometric clustering structure\textemdash i.e. by sampling diversely from each cluster in the ring.

\subsection{Complexity of active learning}

We now comment on the time and space complexity of our algorithm. In general, one would assume that the most expensive step is computing the principal eigenpairs of $L_\mathcal{U}$. However, one key advantage of SSM is that it may provide accurate estimates of the principal eigenvectors of $L$, coinciding with the iterates $X_t$. In particular, 
%if $u$ (line 1 Algorithm~\ref{alg:ssm}) is an estimate of the eigenvector of $L_\mathcal{U}$, 
$u = V \tilde{u}$ is an estimate for the eigenvectors of $L$, if $\tilde{u}$ consists of the eigenvectors of $\tilde{L}$ corresponding to the smallest two eigenvalues. Thus, when iteratively deriving vertices to label via active learning and subsequently solving the graph-based SSL classification problem, we may effectively re-use the previous iteration's estimate of $u$ to do active learning in linear time, comparable to simple, decision-boundary-based margin methods and far more efficient compared to uncertainty uncertainty-based techniques that necessitate full or partial eigenvector decompositions of dense covariance matrices.

\iffalse
\subsection{Transitioning to margin-based active learning}

consider the supervised-unsupervised tradeoff score:
$$
\argmax_{v_i} \lambda \cdot ||2 \cdot U_i \odot \sum_{v_j \in N_i \setminus l}U_j|| - (1-\lambda) \cdot \text{conf}((UQ)_i)
$$
Where $\lambda$ governs the exploration-exploitation tradeoff. I choose lambda according to the following rule:
$$
\lambda_{t+1} = \lambda_t \cdot \mu
$$
where $\mu = \left(\frac{\epsilon}{\lambda_0} \right)^{1/(2k)} \in (0,1)$, $\epsilon = 10^{-8}$, and $k$ is a parameter that depends on the number of clusters in the graph. The idea is that as over time, we switch from exploration to exploitation.
\fi

==> sections/outline.tex <==
%Outline the paper
%first write section headings
%then subsection headings
%then one line summary of each paragraph

\section{Introduction}

\begin{itemize}
\item Introduce semi supervised learning
\item What is the state of the art for graph based semi-supervised learning at low label rates? Laplace learning, Poisson learning, etc.
\item Other notable recent approaches: WNLL, etc.
\item Our contributions: new formulation, a reasonable interpretation, approximate and globally convergent iterative method, numerical results.
\end{itemize}

\section{Preliminaries}
\begin{itemize}
\item Discuss graph SSL learning framework
\item Mention laplace learning algorithms and other relevant methods.
\end{itemize}

\section{Formulation}

\begin{itemize}
\item Start with classic Laplacian Eigenmaps: Solution of a Rayleigh Quotient minimization problem.
\item Introduce the decomposition: Quadratic + affine objective and quadratic + linear  constraints.
\item How can we transform this problem into a more familiar framework? Rescaling simplifies thequadratic constraint and leads to something that looks like a generalization of the trust-region subproblem. 
\item Eliminate constraint on the first moment of $X$. Introduce the projection $P$ onto the orthogonal complement of $1$, the set of centered vectors and the variable substitution $x \gets PX$. The projection is done implicitly.
\item We state the problem, its lagrangian, and the corresponding first order condition.
\item State semidefinite property here or in the algorithm section?
\end{itemize}

\section{Methods}
\subsection{Approximate algorithm}
\begin{itemize}
\item First describe what we will talk about: an approximate method that leads to a feasible solution of the first-order necessary conditions for optimality. Eventually, we'll show that an iterative method is globally convergent in the limit, but good initializations is still extremely important.
\item Describe the approximate algorithm: 3 steps- eigenvector calculation, projection, rescaling/rotation. 
\item Provide interpretation of approximate algorithm using Laplacian SSL / Procrustes alignment.
\end{itemize}

\subsection{SSM}
\begin{itemize}
\item Motivate SSM: why do we need this as an alternative to projected gradient descent? In practice, gradient descent takes a long time and many iterations to converge.
\item Introduce the subspace: span of current iterate, gradient, newton, eigenvectors.
\item How do we compute newton directions for constrained problems? Introduce principle of SQP: solve a linearization of the first order conditions and reference algorithm
\item Why eigenvectors? State convergence result. 
\end{itemize}

\subsection{Experiments}
\begin{itemize}
\item Re-motivate using figure 1- correlation and scatter plots to demonstrate the quadratic spread efffect
\item Point to tables: ssl at low label rates - we consistently outperform relevant methods
\item Imbalanced learning?
\end{itemize}

\section{Conclusion}

\begin{itemize}
\item Review contributions:
\item Novel formulation, approximate algorithm for initialization, globally convergent iterative method, generalization of trust-region subproblem
\end{itemize}

\section{Appendix}
\begin{itemize}
\item Preliminaries
\item Results on the sphere
\item Computational results
\item Convergence
\end{itemize}

==> statements/ssm_convergence.tex <==
\begin{restatable}[Global convergence of SSM]{theorem}{ssm}
\label{thm:ssm_convergence}
A limit $X_*$ of $\{X_1, X_2, \ldots, X_t,\ldots\}$ generated by SSM is a local minmizer of \eqref{eq:cneqi}.
\end{restatable}

==> tables/scaling.tex <==
\begin{table}[h!]
%\vspace{-3mm}
\caption{Scaling behavior as the number of labeled vertices increases beyond the low label rate regime: Average accuracy scores over 10 trials. Standard deviation across trials approaches zero for all methods. We use the publicly available implementation of Poisson Learning~\cite{calder2017consistency}.}
%\vspace{-3mm}
\label{tab:scaling}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lllll}
\toprule
 \# Labels per class &\textbf{500}&\textbf{1000}&\textbf{2000}&\textbf{4000}\\
%\midrule
\midrule
\textbf{MNIST} & & & & \\
Laplace/LP   & \textbf{97.8}    &  97.9   & \textbf{98.1}   &  \textbf{98.3}   \\
%Poisson    & 97.1   &  96.9  &  96.3 &  93.8   \\
Poisson    & 97.1   &  97.2  &  97.2 &  97.2   \\
SSM   &  \textbf{97.8}   &  \textbf{98.0}    &   \textbf{98.1}  &   98.2   \\
\midrule
\textbf{FashionMNIST} & & & & \\
Laplace/LP   & 84.0   &84.7      &85.3      &85.8          \\
%Poisson    & 82.2   &78.9      &74.9       &58.6       \\
Poisson    & 82.2   &82.4      &82.4       &82.4       \\
SSM   &   \textbf{84.3}  &  \textbf{84.8}    &  \textbf{85.9}  &   \textbf{86.1}     \\
%\midrule
%\textbf{CIFAR-10} & & & & \\
%Laplace/LP   & \textbf{72.3}    & \textbf{75.4}      &78.3       & \textbf{80.9}          \\
%Poisson    & 68.8       &69.0      &75.7      &76.2          \\
%SSM    & 72.1  &  75.0  & \textbf{78.7}   &  \textbf{80.9}     \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
